Recurrent Neural Networks for Driver Activity Anticipation via Sensory-Fusion Architecture

Anticipating the future actions of a human is a widely studied problem in robotics that requires spatio-temporal reasoning. In this work we propose a deep learning approach for anticipation in sensory-rich robotics applications. We introduce a sensory-fusion architecture which jointly learns to anticipate and fuse information from multiple sensory streams. Our architecture consists of Recurrent Neural Networks (RNNs) that use Long Short-Term Memory (LSTM) units to capture long temporal dependencies. We train our architecture in a sequence-to-sequence prediction manner, and it explicitly learns to predict the future given only a partial temporal context. We further introduce a novel loss layer for anticipation which prevents over-fitting and encourages early anticipation. We use our architecture to anticipate driving maneuvers several seconds before they happen on a natural driving data set of 1180 miles. The context for maneuver anticipation comes from multiple sensors installed on the vehicle. Our approach shows significant improvement over the state-of-the-art in maneuver anticipation by increasing the precision from 77.4% to 90.5% and recall from 71.2% to 87.4%.

==> maneuver_backup.tex <==
% !TEX root = main.tex

\section{Training the network for maneuver anticipation}
\label{sec:maneuver}
In maneuver anticipation the goal is to anticipate the driver's future maneuver several seconds before it happens~\citep{Jain15,Morris11}. The contextual information for anticipation is extracted from sensors installed in the vehicle. Previous work from Jain et al.~\citep{Jain15} consider the context from a driver facing camera, a camera facing the road in front, a Global Positioning System (GPS), and an equipment for recording the vehicle's dynamics. The overall contextual information from the sensors is grouped into: (i) the context from inside the vehicle, which comes from the driver facing camera and is represented as temporal sequence of features $(\ve{x}_1,...,\ve{x}_T)$; and (ii) the context from outside the vehicle, which comes from remaining sensors and is represented as $(\ve{z}_1,...,\ve{z}_T)$.

 In order to anticipate maneuvers our RNN architecture (Figure~\ref{fig:fusion}) processes temporal context $(\ve{x}_1,...,\ve{x}_t)$ and $ (\ve{z}_1,...,\ve{z}_t)$  at every time step $t$, and outputs softmax probabilities $\ve{y}_t$ for the following five maneuvers:  $\mathcal{M}=$~\{\textit{left turn}, \textit{right turn}, \textit{left lane change}, \textit{right lane change}, \textit{straight driving}\}. We now give an overview of our feature representation and then describe our training procedure.



\iffalse
In maneuver anticipation the goal is to anticipate a vehicle's future maneuver several seconds before it happens~\citep{Jain15,Morris11}. The contextual information for anticipation is extracted from sensors installed in the vehicle. Previous work from Jain et al.~\citep{Jain15} and Morris et al.~\citep{Morris11} consider the context comprising of two sensory streams: (i) $(\ve{x}_1,...,\ve{x}_T)$ represents the driving context inside the vehicle such as the driver's head movements; and (ii) $(\ve{z}_1,...,\ve{z}_T)$ represents the driving context outside the vehicle such as lane or traffic information.
In order to anticipate maneuvers our RNN architecture (Figure~\ref{fig:fusion}) processes temporal context $(\ve{x}_1,...,\ve{x}_t)$ and $ (\ve{z}_1,...,\ve{z}_t)$  at every time step $t$, and outputs softmax probabilities $\ve{y}_t$ for the following five maneuvers:  $\mathcal{M}=$~\{\textit{left turn}, \textit{right turn}, \textit{left lane change}, \textit{right lane change}, \textit{straight driving}\}. We now describe our training procedure and give an overview of our feature representation.
\fi

\begin{figure*}[t]
\centering	
\includegraphics[width=\linewidth]{../Fig/rnn_b4c/sys_fig.png}
\caption{\textbf{Maneuver anticipation pipeline.} Temporal context in maneuver anticipation comes from cameras facing the driver and the road, GPS, and the vehicle's dynamics. (\textbf{a}, \textbf{b} and \textbf{c}) We improve upon the vision pipeline from Jain et al.~\citep{Jain15} by tracking 68 landmark points on the driver's face and including 3D head-pose features. (\textbf{d}) Using Fusion-RNN we combine the sensory streams of features from inside the vehicle (driver facing camera) and outside the vehicle (road camera, GPS, vehicle dynamics).}
\end{figure*}


\subsection{Features}
\label{subsec:features}
\iffalse
We give an overview of the vehicle setup and feature representation from Jain et al.~\citep{Jain15} and describe our feature improvements. The vehicle for maneuver anticipation is equipped with a driver facing camera, a camera facing the road in front, a Global Positioning System (GPS), and an equipment for recording the vehicle's dynamics. The overall contextual information from the sensors is grouped into: (i) the context from inside the vehicle, which comes from the driver facing camera and is represented as temporal sequence of features $(\ve{x}_1,...,\ve{x}_T)$; and (ii) the context from outside the vehicle,  which comes from remaining sensors and is represented as $(\ve{z}_1,...,\ve{z}_T)$.
\fi

We now describe the feature representation of $\ve{x}_t$ and $\ve{z}_t$ from Jain et al.~\citep{Jain15}.
The driver facing camera detects discriminative points on the driver's face and tracks the detected points across frames using KLT tracker~\citep{Shi94}. The tracking generates 2D optical flow trajectories in the plane of image. From these trajectories the horizontal and angular movements of the face are extracted, and these movements are binned into histogram features for every frame. These histogram features are aggregated over 20 frames (i.e. 0.8 seconds of driving) and constitute the feature vector  $\ve{x}_t \in \mathbb{R}^9$. 
Further context for anticipation comes from the camera facing the road, the GPS, 
and the vehicle's dynamics. This is denoted by the feature vector $\ve{z}_t \in \mathbb{R}^6$, and includes the lane information, the road artifacts such as intersections, and the vehicle's speed. 
We refer the reader to Jain et al.~\citep{Jain15} for more information.

\textbf{3D head pose and facial landmark features.} We propose improvements over the features from Jain et al.~\citep{Jain15}. Instead of tracking discriminative points on the driver's face we use Active Appearance Model (AAM)~\citep{Cootes01} and track 68 fixed  landmark points on the driver's face~\citep{Baltrusaitis13}. This offers us two distinct benefits: (i) while discriminative facial points may change from situation to situation, tracking fixed landmarks results in consistent optical flow trajectories; and (ii) it also allows us to estimate 3D head pose of the driver's face by minimizing the error in projection of a generic 3D mesh model of the face w.r.t. the 2D location of landmarks in the image. Including 3D head pose features (yaw, pitch, and roll) with the histogram features generated from optical flow trajectories gives $\ve{x}_t \in \mathbb{R}^{12}$. 

In Section~\ref{experiments} we present results with the features from Jain et al.~\citep{Jain15}, as well as the results with our improved AAM features.

\iffalse
\subsection{Data augmentation and model training}
\label{subsec:augmentation}

Before training our network for maneuver anticipation we add redundancy to the training data by data augmentation. The redundant data acts like a regularizer and reduces the risk of over fitting~\citep{Krizhevsky12,Hannun14}. 
%Data augmentation has been shown to work well on image and speech recognition tasks~\citep{Krizhevsky12,Hannun14}. 
While data augmentation has been well studied for feed-forward networks such as Convolutional Neural Networks~\citep{Krizhevsky12}, it is not yet clear how to augment data for RNNs. We augment data for maneuver anticipation by extracting sub-sequences of temporal context. Given a training example with two temporal sensor streams $\{(\ve{x}_1,...,\ve{x}_T),(\ve{z}_1,...,\ve{z}_T),y\}$, we uniformly randomly sample multiple sub-sequences $\{(\ve{x}_i,...,\ve{x}_j),(\ve{z}_i,...,\ve{z}_j),y | 1 \leq i < j \leq T\}$ as additional training examples. It is important to realize that data augmentation only adds redundancy and does not rely on any external source of new information. 
\iffalse
Data augmentation involves increasing the size of training data by adding new examples that are either synthetically generated, or obtained through various \textit{augmentation} operations on the training data set. Since the number of parameters in a deep network is typically more than the number of training examples, data augmentation reduces the risk of over fitting. It has been shown to work well on image and speech recognition tasks~\citep{Krizhevsky12,Hannun14}. While data augmentation has been well studied for feed-forward networks such as Convolutional Neural Networks~\citep{Krizhevsky12}, it is not yet clear how to augment data for RNNs.  In order to train our network for maneuver anticipation we augment the training data by extracting sub-sequences of temporal context. Given a training example with two temporal sensor streams $\{(\ve{x}_1,...,\ve{x}_T),(\ve{z}_1,...,\ve{z}_T),y\}$, we uniformly randomly sample multiple sub-sequences $\{(\ve{x}_i,...,\ve{x}_j),(\ve{z}_i,...,\ve{z}_j),y | 1 \leq i < j \leq T\}$ as additional training examples.	
\fi

On the augmented data set we train the network described in Section~\ref{sec:sensor-fusion-rnn}. We use RMSprop gradients which have been shown to work well on training deep networks~\citep{Dauphin15}, and we keep the step size fixed at $1e^{-4}$. We experimented with different variants of softmax loss, however, our proposed loss-layer with exponential growth Eq.~\eqref{eq:loss} works best for anticipation (see Section~\ref{experiments} for details).
\fi


\iffalse
We use Stochastic Gradient Descent (SGD)~\citep{Bottou10} to minimize the exponentially growing loss function. We use RMSprop gradients in SGD which has been shown to work well on training deep networks~\citep{Dauphin15}, and we keep the step size fixed at $1e^{-4}$. We experimented with different variants of softmax loss, however, our proposed loss-layer with exponential decay~\eqref{eq:loss} works best for anticipation. See Section~\ref{experiments} for details.
\todo{move equation~\eqref{eq:loss} to the para describing the loss?}
\fi

